Online Non-Monotone DR-submodular Maximization

In this paper, we study fundamental problems of maximizing DR-submodular continuous functions that have real-world applications in the domain of machine learning, economics, operations research and communication systems. It captures a subclass of non-convex optimization that provides both theoretical and practical guarantees. Here, we focus on minimizing regret for online arriving non-monotone DR-submodular functions over different types of convex sets: hypercube, down-closed and general convex sets. First, we present an online algorithm that achieves a $1/e$-approximation ratio with the regret of $O(T^{2/3})$ for maximizing DR-submodular functions over any down-closed convex set. Note that, the approximation ratio of $1/e$ matches the best-known guarantee for the offline version of the problem. Moreover, when the convex set is the hypercube, we propose a tight 1/2-approximation algorithm with regret bound of $O(\sqrt{T})$. Next, we give an online algorithm that achieves an approximation guarantee (depending on the search space) for the problem of maximizing non-monotone continuous DR-submodular functions over a \emph{general} convex set (not necessarily down-closed). To best of our knowledge, no prior algorithm with approximation guarantee was known for non-monotone DR-submodular maximization in the online setting. Finally we run experiments to verify the performance of our algorithms on problems arising in machine learning domain with the real-world datasets.

==> related.tex <==
%!TEX root = main.tex

% summary about offline (DR)-submodular minimization and maximization.

\section{Related Work}


In this section, we give a summary on 
%submodular maximization and on 
DR-submodular maximization 
%as it is closely related to the former.
%Submodular optimization has been widely studied for decades \cite{NemhauserWolsey78:An-analysis-of-approximations,Fujishige05:Submodular-functions}. 
The domain has been investigated more extensively 
in recent years due to its numerous applications in the field of statistics and machine learning, for example 
active learning \cite{GolovinKrause11:Adaptive-submodularity:}, 
viral makerting \cite{KempeKleinberg03:Maximizing-the-spread}, 
network monitoring \cite{Gomez-RodriguezLeskovec10:Inferring-networks}, 
document summarization \cite{LinBilmes11:A-class-of-submodular},
crowd teaching \cite{SinglaBogunovic14:Near-Optimally-Teaching}, 
feature selection \cite{ElenbergKhanna18:Restricted-strong}, 
deep neural networks \cite{ElenbergDimakis17:Streaming-weak}, 
diversity models \cite{DjolongaTschiatschek16:Variational-inference} and
recommender systems \cite{GuilloryBilmes11:Simultaneous-Learning}. 


\paragraph{Offline setting.}
%
%In standard approximation theory, the problem of minimization a submodular function is polynomial solvable~\cite{Schrijver00:A-combinatorial-algorithm,IwataFleischer01:A-combinatorial-strongly}. 
%
%On the other hand, the problem of maximizing an unconstrained submodular function is NP-hard.  
%%
%Thus over the year, several approximation algorithms have been developed in offline settings, for example $(1/2)$-approximation algorithm for unconstrained domains~\cite{BuchbinderFeldman15:A-tight-linear,BuchbinderFeldman18:Deterministic-algorithms}, 
%$(1-1/e)$-approximation algorithm for monotone smooth submodular functions
%\cite{CalinescuChekuri11:Maximizing-a-monotone,ChekuriJayram15:On-multiplicative-weight}, 
%$\left(1/e\right)$-approximation algorithm for non-monotone submodular functions on down-closed polytopes \cite{FeldmanNaor11:A-unified-continuous,ChekuriJayram15:On-multiplicative-weight}.
%
%The continuous extensions of submodular functions such as the multilinear relaxation and the softmax extension,  play a crucial role in submodular maximization.  See \cite{Bachothers13:Learning-with} for a survey on connections and applications in machine learning. 
%%
%These extensions belong to a broad class of DR-submodular functions. 
%
\cite{BianMirzasoleiman17:Guaranteed-Non-convex} considered the problem of maximizing monotone DR-functions subject to a down-closed convex domain and showed that the greedy method proposed by \cite{CalinescuChekuri11:Maximizing-a-monotone}, (a variant of well-known Frank-Wolfe algorithm in convex optimization), guarantees a $(1-1/e)$-approximation.
%
However, it has been observed by \cite{HassaniSoltanolkotabi17:Gradient-methods} 
that the greedy method is not robust in stochastic settings
(where only unbiased estimates of gradients are available). Subsequently, they
showed that the gradient methods achieve $(1/2)$-approximation for monotone functions in stochastic settings. 
\cite{MokhtariHassani18:Conditional-Gradient} proposed the sample-efficient variance reduction technique for
projection-free algorithms. Their method achieves an $(1-1/e)$-approximation guarantee for monotone and continuous DR-submodular functions over a general convex domain. 

%Although these variance reduction techniques have enjoyed success in the offline setting, they have yet to be as extensively applied in the online setting

The problem of maximizing non-monotone DR-submodular functions is much harder. 
%
Very recently, \cite{BianBuhmann18:Optimal-DR-Submodular} and \citet{NiazadehRoughgarden18:Optimal-Algorithms}
have independently presented algorithms with the same approximation guarantee of $(1/2)$ for the problem of 
unconstrained non-monotone DR-submodular maximization ($\mathcal{K} = [0,1]^{n}$).
These algorithms are inspired by the bi-greedy algorithm in \cite{BuchbinderFeldman15:A-tight-linear,BuchbinderFeldman18:Deterministic-algorithms}. 
\cite{BianLevy17:Non-monotone-Continuous} made a further step by providing an 
$(1/e)$-approximation algorithm where the domains are down-closed convex. 
\citet{MokhtariHassani18:Conditional-Gradient} also presented an  algorithm that achieve $(1/e)$ for non-monotone continuous DR-submodular function over a down-closed convex domain that uses only stochastic gradient estimates.
Remark that when aiming for approximation algorithms (in polynomial time), the restriction to down-closed polytopes is unavoidable.
Specifically, \cite{Vondrak13:Symmetry-and-approximability} proved that any algorithm for the problem over a non-down-closed domain that guarantees a constant approximation must require exponentially many value queries to the function. More specifically, he considers the problem of maximizing a non negative submodular function over a collection of bases in a matroid, and shows that any constant approximation requires an exponential number of queries to $f$ and therefore an exponential running time.  Keeping this mind, \cite{durr-thang:2019} presented an algorithm that achieves $\left(\frac{1-\min_{\vect{x} \in \mathcal{K}} \|\vect{x}\|_{\infty} }{3\sqrt{3}} \right)$-approximation for non-monotone DR-submodular function over a general convex domain (not necessarily down-closed convex domain).




% summary about online (DR)-submodular minimization and maximization.
\paragraph{Online setting.}
Chen et al.~\cite{ChenHassani18:Online-continuous} considered the online problem of maximizing monotone smooth DR-submodular functions and provided an algorithm that achieves a $\bigl(1-1/e, O(\sqrt{T})\bigr)$-regret. 
For the general problem of monotone DR-submodular functions functions (not necessarily smooth), Chen et al.~\cite{ChenHassani18:Online-continuous} proved that the online gradient ascent algorithm 
guarantees a $\bigl(1/2,O(\sqrt{T})\bigr)$-regret using unbiased stochastic gradient estimates. For monotone DR-submodular functions, Zhang et al.~\cite{Zhang:2019} presented an algorithm that reduces the number of per-function gradient evaluations from $T^{3/2}$ in \cite{ChenHassani18:Online-continuous} to $1$ and achieves the same approximation ratio of $(1-1/e)$. More importantly, they presented a bandit algorithm for maximizing monotone DR-submodular function over a general convex set that achieves in expectation $(1-1/e)$ approximation ratio with regret $O(T^{8/9})$.
\cite{RoughgardenWang18:An-Optimal-Algorithm} have studied the unconstrained non-monotone (discrete) submodular maximization and provided an optimal $(1/2)$-approximation factor with $O(\sqrt{T})$ regret.  
Recently, \cite{Thang:2019b} presented an online algorithm that achieves $\left(\frac{1-\min_{\vect{x} \in \mathcal{K}} \|\vect{x}\|_{\infty} }{3\sqrt{3}} \right)$-approximation for non-monotone DR-submodular function over a general convex domain  with $O(T/\ln T)$-regret. Their algorithm uses stochastic estimates of gradients similar to the one mentioned in~\cite{ChenHassani18:Online-continuous}. 



%
%Maximizing submodular (set) functions have been considered in the competitive analysis model. 
%\citet{Feige11:Non-monotone-sub-func} considered the setting where given a non-monotone submodular reward function, 
%elements arrive in online fashion and the algorithm at each time step makes an irrevocable decision 
%of either selecting or rejecting the newly arrived element (without any constraint). 
%The objective is to maximize the reward incurred on the set of chosen elements. 
%They presented a simple $(1/4)$-competitive algorithm for the problem.  
%Later on, \citet{Buchbinder15:OSM} showed competitive bound of $(1/e)$ in the preemptive model 
%where the algorithm is allowed to discard/reject the previously selected elements. 
%They also proved that no randomized algorithm can have better competitive ratio than $(4/5)$. 


%An important research agenda is to design algorithms with performance guarantees 
%in terms of regret and approximation for non-convex functions in general and for non-monotone continuous DR-submodular functions. 


%\paragraph{Bandit setting.} In the bandit setting, submodular optimization has been studied for minimization problems \cite{HazanKale12:Online-submodular}. However, no non-trivial approximation guarantee for non-monotone submodular maximization is known in the bandit settings. \textcolor{red}{To add Lin Chen's NIPS results}

% summary about bandit (DR)-submodular minimization and maximization.
%\paragraph{Bandit submodular optimization.}


 











==> vee.tex <==
%!TEX root = main.tex


\section{Online Vee Oracle} 

In this section, we design an online algorithm that maximizes $\sum_{t=1}^T \langle \vect{a}^t, \vect{c}^t \vee \vect{x}^t \rangle$ such that $\vect{c}^t, \vect{x}^t \in {\cal K}$ and $\vect{c}^t$ is known a prori. More specifically, at each time $t$, the online algorithm knows $\vect{c}^t$ in advance and selects a vector $\vect{x}^t$. Subsequently, the adversary reveals a vector $\vect{a}^t \in \mathbb{R}^{n}$  and the algorithm receives a reward $\langle \vect{a}^t, \vect{c}^t \vee \vect{x}^t \rangle$. The goal is to maximize the total reward over a time horizon $T$. %Note that, only $\vect{x}^t$'s are the decision variables.


\paragraph{Discretization and lifting.}
Let $\mathcal{L}$ be a lattice such that $\mathcal{L} = \{0, \frac{1}{M}, \frac{2}{M}, \ldots,  \frac{\ell}{M}, \ldots, 1\}^{n}$ where $0 \leq \ell \leq M$ for some parameter $M$ (to be defined later). 
Note that each $x_{i} = \frac{\ell}{M}$ for $1 \leq \ell \leq M$ 
can be uniquely represented by a vector $\vect{y}_{i} \in \{0,1\}^{M}$ 
such that $y_{i1} = \ldots = y_{i\ell} = 1$ and $y_{i,\ell+1} = \ldots = y_{i,M} = 0$. 
Based on this view, we lift the discrete set $\mathcal{K} \cap \mathcal{L}$ to the $(n \times M)$-dim space.
Specifically, define a \emph{lifting} map $m: \mathcal{K} \cap \mathcal{L} \rightarrow \{0,1\}^{n \times M}$
such that each point $(x_{1}, \ldots, x_{n}) \in \mathcal{K} \cap \mathcal{L}$
maps to an unique point $(y_{10}, \ldots, y_{1M}, \ldots, y_{n0}, \ldots, y_{nM}) \in \{0,1\}^{n \times M}$
where $y_{i1} = \ldots = y_{i\ell} = 1$ and $y_{i,\ell+1} = \ldots = y_{i,M} = 0$ iff $x_{i} = \frac{\ell}{M}$ for $1 \leq \ell \leq M$.
Define $\widetilde{\mathcal{K}}$ be the set 
$\{ \vect{1}_{X} \in  \{0,1\}^{n \times M}: \vect{1}_{X} = m(\vect{x}) \text{ for some } \vect{x} \in \mathcal{K} \cap \mathcal{L} \}$.
Observe that $\widetilde{\mathcal{K}}$ is a subset of discrete points $\{0,1\}^{n \times M}$. 
Let $\mathcal{C} := \texttt{conv}(\widetilde{\mathcal{K}})$ be the convex hull of $\widetilde{\mathcal{K}}$.





In our algorithm, at every time $t$, we will output $\vect{x}^{t} \in \mathcal{L}$. In fact, we will reduce the original problem to 
a linear optimization problem in the $(n \times M)$-dim space. Given $\vect{c}^{t} \in {\cal K}$, we round every coordinate $c^{t}_{i}$ 
for $1 \leq i \leq n$ to the largest multiple of $\frac{1}{M}$ which is smaller than $c^{t}_{i}$. Specifically, the rounded vector 
$\overline{\vect{c}}^{t}$ has the $i^{th}$-coordinate $\bar{c}^{t}_{i} = \frac{\ell}{M}$ where 
$\frac{\ell}{M} \leq c^{t}_{i} \leq  \frac{\ell+1}{M}$. Vector $\overline{\vect{c}}^{t} \in \mathcal{L}$ and also $\overline{\vect{c}}^{t} \in \mathcal{K}$ (since $\overline{\vect{c}}^{t} \leq \vect{c}^{t}$ and $\mathcal{K}$ is down-closed). Denote 
$\vect{1}_{C^{t}} = m(\overline{\vect{c}}^{t})$. Besides, for each vector $\vect{a}^{t} \in \mathbb{R}^{n}$, 
define its correspondence $\widetilde{\vect{a}}^{t} \in \mathbb{R}^{n \times M}$ such that $\widetilde{a}^{t}_{i,j} = \frac{1}{M} a^t_i$ for all $1 \leq i \leq n$ and $1 \leq j \leq M$. 
Observe that $\langle \vect{a}^{t}, \overline{\vect{c}}^{t} \rangle = \langle \widetilde{\vect{a}}^{t}, \vect{1}_{C^{t}} \rangle$.


\begin{algorithm}[h]
\begin{flushleft}
\textbf{Input}:  A convex set $\mathcal{K}$, a time horizon $T$.
\end{flushleft}
\vspace{-0.4cm}
\begin{algorithmic}[1]
\STATE Let $\mathcal{L}$ be a lattice in $[0,1]^{n}$ and denote the convex set $\mathcal{C} := \texttt{conv}(\widetilde{\mathcal{K}})$.
\STATE Initialize arbitrarily $\vect{x}^{1} \in \mathcal{K} \cap \mathcal{L}$ and 
	$\vect{y}^{1} = \vect{1}_{X^{1}} = m(\vect{x}^{1}) \in \widetilde{\mathcal{K}}$.
\FOR {$t = 1$ to $T$}	 		
		%
		\STATE Observe $\vect{c}^{t}$, compute $\vect{1}_{C^{t}} = m(\overline{\vect{c}}^{t})$.
		\STATE Play $\vect{x}^{t}$.
		\STATE Observe $\vect{a}^{t}$ (so compute $\widetilde{\vect{a}}^{t}$) 
			and receive the reward $\langle \vect{a}^{t}, \vect{x}^{t} \rangle$.
		\STATE Update: $\vect{y}^{t+1} \gets \texttt{update}_{\mathcal{C}}(\vect{y}^{t}; \widetilde{\vect{a}}^{t'} \circ (\vect{1} - \vect{1}_{C^{t'}}): t' \leq t)$
			where $\circ$ denote the element-wise multiplication.
		\STATE Round: $\vect{1}_{X^{t+1}} \gets \texttt{round}(\vect{y}^{t+1})$.
		\STATE Compute $\vect{x}^{t+1} = m^{-1}(\vect{1}_{X^{t+1}})$.
\ENDFOR
\end{algorithmic}
\caption{Online algorithm for vee learning}
\label{algo:vee}
\end{algorithm}

\paragraph{Update scheme.}
In the algorithm, we use a procedure \texttt{update}. This procedure takes arguments as the convex set 
$\mathcal{C}$, the current vector $\vect{y}^{t}$, the gradients of previous time steps $\widetilde{\vect{a}}^{t} \circ (\vect{1} - \vect{1}_{C^{t}})$ and outputs the next vector $\vect{y}^{t+1}$. One can use different update strategies, in particular 
the gradient-based updates or the family of follow-the-leader strategies. 
\begin{align*}
	\vect{y}^{t+1} &\gets \texttt{Proj}_{\mathcal{C}}\left( \vect{y}^{t} - \eta \cdot \widetilde{\vect{a}}^{t} \circ (\vect{1} - \vect{1}_{C^{t}}) \right)
		& \qquad \text{(Gradient Descent)}  \\
	%
	\vect{y}^{t+1} &\gets \arg \min_{\mathcal{C}} \biggl\{ \eta \sum_{t'=1}^{t} \langle \widetilde{\vect{a}}^{t'} \circ (\vect{1} - \vect{1}_{C^{t'}}), \vect{y} \rangle + \vect{n}^{T} \cdot \vect{y} \biggr\}
		& \qquad \text{(Follow-the-perturbed-leader)}
\end{align*}

\paragraph{Rounding scheme.}
Besides, in the algorithm, we use additionally a procedure \texttt{round} in order to transform a solution $\vect{y}^{t}$
in the convex set $\mathcal{C}$ of dimension $n \times M$ to an integer point in $\widetilde{\mathcal{K}}$. 
Specifically, given $\vect{y}^{t} \in \texttt{conv}(\widetilde{\mathcal{K}})$, we round $\vect{y}^{t}$ to $\vect{1}_{X^{t}} \in \widetilde{\mathcal{K}}$. \thang{It'd better to round using the (approximate) Carathéodory's theorem}
Observe that $\vect{y}^{t} \in \texttt{conv}(\widetilde{\mathcal{K}})$ so $y^t_{ij} \geq y^t_{ij'}$ for every $1 \leq j \leq j' \leq M$ 
and for every $i$. At time $t$, we are given $\vect{1}_{C^{t}} \in \widetilde{\mathcal{K}}$.  
First, fix a coordinate $1 \leq i \leq n$, round $(y_{i1}, \ldots, y_{iM})$ to a vector $Y_{i}$ of form $1^{j} 0^{M-j}$ 
with probability $y_{i,j} - y_{i,j+1}$ for every $0 \leq j \leq M$ with convention that $y_{i,0} = 1$ and $y_{i,M+1} = 0$. 
Remark that it is well-defined since $y_{i,j-1} \geq y_{i,j}$ 
for $1 \leq j \leq M$ and the total probability equals 1. 
By that rounding, 
$$
\mathbb{E}[Y_{i}] = \sum_{j=0}^{M} (y_{i,j} - y_{i,j+1}) \cdot (\underbrace{1, \ldots, 1}_{j}, \underbrace{0, \ldots, 0}_{M- j}) 
=  (y_{i1}, \ldots, y_{iM}).
$$ 
Now, it remains to round independently for very $1 \leq i \leq n$. 
Concretely, round $\vect{y}^{t}$ to $(1^{j_{1}} 0^{M-j_{1}}, \ldots, 1^{j_{n}} 0^{M-j_{n}})$ $\in \widetilde{\mathcal{K}}$ with probability
$\prod_{i=1}^{n} \mathbb{P}[Y_{i} = 1^{j_{i}} 0^{M-j_{i}}]$. 


%Now consider the following linear optimization problem. 
%At every time $t$, given $\vect{1}_{C^{t}} \in \{0,1\}^{n\times M}$, 
%one needs to choose $\vect{x}^{t} \in \texttt{conv}(\widetilde{\mathcal{K}})$. Subsequently, a linear function 
%$\widetilde{\vect{a}}^{t}$ is released and the algorithm receives the reward 
%$\langle \widetilde{\vect{a}}^{t} - \widetilde{\vect{a}}^{t} \circ \vect{1}_{C^{t}}, \vect{x}^{t} \rangle$. 
%The objective is to minimize the regret. 



\begin{lemma}
\label{vee-learning}
Assume that $\|\vect{a}^{t}\| \leq G$ for all $t$ and the update scheme is either the gradient ascent update or 
the follow-the-perturbed-leader update. Then, using the lattice $\mathcal{L}$ with parameter 
$M= (T/n)^{1/4}$, Algorithm~\ref{algo:vee} achieves a regret bound of 
$O\bigl(G (n T)^{3/4}\bigr)$.
\end{lemma}
%
%
\begin{proof}
Observe that  $\vect{y}^{t}$ be the solution of the online linear optimization problem at time $t$ where 
the reward function at time $t$ is $\langle \widetilde{\vect{a}}^{t} \circ (\vect{1} - \vect{1}_{C^{t}}), \cdot  \rangle$.  

First, by the construction, we have:
\begin{align*}
m(\overline{\vect{c}}^{t} \vee \vect{x}^{t}) &= m(\overline{\vect{c}}^{t}) \vee m(\vect{x}^{t}) = \vect{1}_{C^{t}} \vee \vect{1}_{X^{t}} \\
%
\langle \vect{a}^{t}, \overline{\vect{c}}^{t}  \vee \vect{x}^{t} \rangle &= 
 \langle \widetilde{\vect{a}}^{t}, \vect{1}_{C^{t}} \vee \vect{1}_{X^{t}} \rangle
\end{align*}
%
%
%
Therefore, 
$$
\sum_{t = 1}^{T} \E \bigl[ \langle \vect{a}^{t}, \overline{\vect{c}}^{t}  \vee \vect{x}^{t} \rangle \bigr ]
= \sum_{t = 1}^{T} \E \bigl[  \langle \widetilde{\vect{a}}^{t}, \vect{1}_{C^{t}} \vee \vect{1}_{X^{t}} \rangle  \bigr ]
$$ 
%
%
%
%
Besides, for every vector $\vect{1}_{C}$ and vector $\vect{y} \in [0,1]^{n \times M}$, the following identity always holds: 
$\vect{1}_{C} \vee \vect{y} = \vect{y} + \vect{1}_{C} \circ (\vect{1} - \vect{y})$.
Therefore, for every vector $\vect{y} \in [0,1]^{n \times M}$,
\begin{align}	\label{eq:vee1}
 \langle \widetilde{\vect{a}}^{t}, \vect{1}_{C^{t}} \vee\vect{y} \rangle
 &=  \langle \widetilde{\vect{a}}^{t}, \vect{y} + \vect{1}_{C^{t}} \circ (\vect{1} - \vect{y}) \rangle
 = \langle \widetilde{\vect{a}}^{t}, \vect{y} \circ (\vect{1} - \vect{1}_{C^{t}}) \rangle
 	+ \langle \widetilde{\vect{a}}^{t},  \vect{1}_{C^{t}} \rangle	\notag \\
%
&=  \langle \widetilde{\vect{a}}^{t} \circ (\vect{1}- \vect{1}_{C^{t}}), \vect{y}  \rangle
 	+ \langle \widetilde{\vect{a}}^{t},  \vect{1}_{C^{t}} \rangle
\end{align}
%
%
%
%
%
Note that the last term $\langle \widetilde{\vect{a}}^{t},  \vect{1}_{C^{t}} \rangle$ is independent of the decision at time $t$. 
By linearity of expectation, we have
%
%
\begin{align}	\label{eq:vee2}
\sum_{t = 1}^{T} \E \bigl[ \langle \vect{a}^{t}, \overline{\vect{c}}^{t}  \vee \vect{x}^{t} \rangle \bigr ]
&= \sum_{t = 1}^{T} \E \bigl[  \langle \widetilde{\vect{a}}^{t} \circ (\vect{1} - \vect{1}_{C^{t}}), \vect{1}_{X^{t}}  \rangle
 	+ \langle \widetilde{\vect{a}}^{t},  \vect{1}_{C^{t}} \rangle  \bigr ] 		\notag \\
%
&= \sum_{t = 1}^{T}  \langle \widetilde{\vect{a}}^{t} \circ (\vect{1} - \vect{1}_{C^{t}}), \vect{y}^{t}  \rangle
 	+ \sum_{t = 1}^{T} \langle \widetilde{\vect{a}}^{t},  \vect{1}_{C^{t}} \rangle. 
\end{align}
%
%
Let $\vect{x}^{*}$ be the optimal solution in hindsight for the online vee learning problem. 
Let $\overline{\vect{x}}^{*}$ be the rounded solution of $\vect{x}^{*}$ onto the lattice $\mathcal{L}$. 
Denote $\vect{1}_{X^{*}} = m(\overline{\vect{x}}^{*})$.
By (\ref{eq:vee1}) and (\ref{eq:vee2}), we have 
%
\begin{align*}
\sum_{t = 1}^{T} \E \bigl[ \langle \vect{a}^{t}, \overline{\vect{c}}^{t}  \vee \vect{x}^{t} \rangle \bigr ]
- \sum_{t = 1}^{T} \langle \vect{a}^{t}, \overline{\vect{c}}^{t}  \vee \overline{\vect{x}}^{*} \rangle
= \sum_{t = 1}^{T} \E \bigl[ \langle \widetilde{\vect{a}}^{t} \circ (\vect{1} - \vect{1}_{C^{t}}), \vect{y}^{t} - \vect{1}_{X^{*}} \rangle \bigr ]
\geq - O(nMG\sqrt{T})
\end{align*}
%
%
%
%
where the last inequality is due to the regret bound of the gradient descent or the follow-the-perturbed-leader algorithms. 
Combining with the Lipschitz property, we have 
%
%
\begin{align*}
\sum_{t = 1}^{T} &\E \bigl[ \langle \vect{a}^{t}, \vect{c}^{t}  \vee \vect{x}^{t} \rangle \bigr ]
- \sum_{t = 1}^{T} \langle \vect{a}^{t}, \vect{c}^{t}  \vee \vect{x}^{*} \rangle \\
&=
\sum_{t = 1}^{T} \E \bigl[ \langle \vect{a}^{t}, \vect{c}^{t}  \vee \vect{x}^{t} \rangle \bigr ]
- \sum_{t = 1}^{T} \langle \vect{a}^{t}, \overline{\vect{c}}^{t}  \vee \vect{x}^{t} \rangle
+\sum_{t = 1}^{T} \E \bigl[ \langle \vect{a}^{t}, \overline{\vect{c}}^{t}  \vee \vect{x}^{t} \rangle \bigr ]
- \sum_{t = 1}^{T} \langle \vect{a}^{t}, \overline{\vect{c}}^{t}  \vee \overline{\vect{x}}^{*} \rangle \\
	&\qquad +\sum_{t = 1}^{T} \E \bigl[ \langle \vect{a}^{t}, \overline{\vect{c}}^{t}  \vee \overline{\vect{x}}^{*} \rangle \bigr ]
	- \sum_{t = 1}^{T} \langle \vect{a}^{t}, \vect{c}^{t}  \vee \overline{\vect{x}}^{*} \rangle 
	+\sum_{t = 1}^{T} \E \bigl[ \langle \vect{a}^{t}, \vect{c}^{t}  \vee \overline{\vect{x}}^{*} \rangle \bigr ]
	- \sum_{t = 1}^{T} \langle \vect{a}^{t}, \vect{c}^{t}  \vee \vect{x}^{*} \rangle \\
%
&\geq - O(nMG\sqrt{T}) - O(T G\frac{\sqrt{n}}{M}).
\end{align*}
Choosing $M = (T/n)^{1/4}$, one gets the regret bound of $O\bigl(G(nT)^{3/4}\bigr)$.
\end{proof}


















